A Continuous Benchmarking Infrastructure for High-Performance Computing Applications

For scientific software, especially those used for large-scale simulations, achieving good performance and efficiently using the available hardware resources is essential. It is important to regularly perform benchmarks to ensure the efficient use of hardware and software when systems are changing and the software evolves. However, this can become quickly very tedious when many options for parameters, solvers, and hardware architectures are available. We present a continuous benchmarking strategy that automates benchmarking new code changes on high-performance computing clusters. This makes it possible to track how each code change affects the performance and how it evolves.

==> util/commands.tex <==
\usepackage{subcaption}
\usepackage[utf8]{inputenc}
\usepackage[dvipsnames]{xcolor}
\usepackage{graphicx}
\RequirePackage{soul}
\usepackage{acro}
\usepackage{fontawesome}
\usepackage{orcidlink}
\usepackage{multirow}
\setlength{\marginparwidth}{2cm}
\usepackage{todonotes}

\usepackage{hyperref}
\usepackage{acro}
\DeclareAcronym{cb}{short=CB, long=continuous benchmarking}
\DeclareAcronym{ci}{short=CI, long=continuous integration}
\DeclareAcronym{cicd}{short=CI/CD, long=Continuous Integration/Continuous Deployment}
\DeclareAcronym{cx}{short={C\textit{X}}, long={Continuous \textit{X}}}
\DeclareAcronym{hpc}{short=HPC, long=High-Performance Computing}
\DeclareAcronym{vcs}{short=VCS, long=version control system}
\DeclareAcronym{lbm}{short=LBM, long=Lattice Boltzmann Method}
\DeclareAcronym{rse}{short=RSE, long=Research Software Engineering}
\DeclareAcronym{bssw}{short=BSSw, long=Better Scientific Software}
\DeclareAcronym{flop}{short=FLOP, long=Floating Point Operation}
\DeclareAcronym{flops}{short=FLOP/s, long=Floating Point Operation per Second}
\DeclareAcronym{tts}{short=TTS, long=Time to Solution}
\DeclareAcronym{tsdb}{short=TSDB, long=Time Series Database}
\DeclareAcronym{rve}{short=RVE, long=representative volume element}
\DeclareAcronym{cfd}{short=CFD, long=computational fluid dynamics}
\DeclareAcronym{fair}{short=FAIR, long={Findable, Accessible, Interoperable, and Reusable}}
\DeclareAcronym{mlups}{short=MLUP/s, long={Mega Lattice Updates per Second}}
\DeclareAcronym{xSDK}{short=xSDK, long={Extreme-scale Scientific Software Development Kit}}
\DeclareAcronym{mpi}{short=MPI, long={Message Passing Interface}}
\DeclareAcronym{openmpi}{short=OpenMP, long=Open Multi-Processing}
\DeclareAcronym{bddc}{short=BDDC, long={Balancing Domain Decomposition by Constraints}}
\DeclareAcronym{pdf}{short=PDF, long={particle distribution function}}
\DeclareAcronym{fslbm}{short=FSLBM, long={free-surface lattice Boltzmann method}}
\DeclareAcronym{ilu}{short=ILU, long={incomplete Lower Upper factorization}}



\newcommand{\gl}{\textit{GitLab}}
\newcommand{\gf}{\textit{Grafana}}
\newcommand{\idb}{\textit{InfluxDB}}
\newcommand{\fl}[1]{\footnote{\url{#1}}}
\newcommand{\nhr}{\textit{NHR@FAU}}
\newcommand{\kadi}{\textit{Kadi4Mat}}
\newcommand{\lwd}{\textit{likwid}}
\newcommand{\ms}{\textit{machine\-state}}
\newcommand{\fe}{\textit{FE2TI}}
\newcommand{\wlb}{\textsc{waLBerla}}
\newcommand{\yml}{\textit{YAML}}
\newcommand{\ncu}{\textit{Nvidia Nsight Compute}}
\newcommand{\skx}{\textit{Intel Xeon Skylake Gold 6148 CPU}}
\newcommand{\icx}{\textit{Intel Xeon Icelake Platinum 8360Y CPU}}
\newcommand{\rome}{\textit{AMD EPYC 7452 Rome CPU}}
\newcommand{\genoa}{\textit{AMD EPYC 9354 Genoa CPU}}

\usepackage{listings}
\newcommand\YAMLcolonstyle{\color{red}\mdseries}
\newcommand\YAMLkeystyle{\color{black}\bfseries}
\newcommand\YAMLvaluestyle{\color{blue}\mdseries}

\definecolor{ocean}{HTML}{07575b}
\definecolor{wave}{HTML}{66A5AD}
\definecolor{seafoam}{HTML}{C4DFE6}
\definecolor{processblue}{cmyk}{0.96,0,0,0}

\lstset{ % General setup for the package
	basicstyle=\small,
	backgroundcolor=\color{seafoam!20},
	numbers=left,
	numberstyle=\footnotesize,
	frame=tb,
	tabsize=2,
	columns=fixed,
	showstringspaces=false,
	showtabs=false,
	keepspaces,
	commentstyle=\color{gray},
	keywordstyle=\color[HTML]{1d741b},
	captionpos=t,
}


\makeatletter

\newcommand\language@yaml{yaml}

\expandafter\expandafter\expandafter\lstdefinelanguage
\expandafter{\language@yaml}
{
keywords={true,false,null,y,n,tags,variables,script},
keywordstyle=\color{darkgray}\bfseries,
basicstyle=\YAMLkeystyle,                                 % assuming a key comes first
sensitive=false,
comment=[l]{\#},
morecomment=[s]{/*}{*/},
commentstyle=\color{purple}\ttfamily,
stringstyle=\YAMLvaluestyle\ttfamily,
moredelim=[l][\color{orange}]{\&},
moredelim=[l][\color{magenta}]{*},
moredelim=**[il][\YAMLcolonstyle{:}\YAMLvaluestyle]{:},   % switch to value style at :
morestring=[b]',
morestring=[b]",
literate =    {---}{{\ProcessThreeDashes}}3
{>}{{\textcolor{red}\textgreater}}1
{|}{{\textcolor{red}\textbar}}1
{\ -\ }{{\mdseries\ -\ }}3,
}

% switch to key style at EOL
\lst@AddToHook{EveryLine}{\ifx\lst@language\language@yaml\YAMLkeystyle\fi}
\makeatother

\newcommand\ProcessThreeDashes{\llap{\color{cyan}\mdseries-{-}-}}

\renewcommand{\figureautorefname}{Fig.}
\renewcommand{\tableautorefname}{Tab.}
\renewcommand{\sectionautorefname}{Sec.}
\renewcommand{\subsectionautorefname}{Sec.}
\renewcommand{\subsubsectionautorefname}{Sec.}
\renewcommand{\equationautorefname}{Eq.}

\RequirePackage{tikz}
\usetikzlibrary{positioning,calc,decorations.pathreplacing,shapes,arrows.meta,decorations.markings,quotes,shapes.geometric,spy}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}
\usepgfplotslibrary{groupplots,dateplot,fillbetween}
\usetikzlibrary{arrows,arrows.meta,patterns,shapes.arrows,calc,angles,quotes,babel}
\usetikzlibrary{calc,angles,quotes}

\newlength\figureheight
\newlength\figurewidth
\newlength\mdist     % distance of measure line and object
\newlength\radius    % radius of the Taylor bubble in the setup figure

